SAPD: Learning from Agent Experience without Environment Interaction

Scaling the training of Large Language Model (LLM) agents typically requires a large collection of executable environments, whose construction, maintenance, and operation constrain the expansion of training experience. Existing offline trajectories offer an opportunity to reuse interaction experience, yet effectively refining the current policy without revisiting these environments remains challenging: supervised fine-tuning (SFT) can lead to catastrophic forgetting, while online reinforcement learning requires real-time interaction with the environment. To address this challenge, we propose Step-Advantage Policy Distillation (SAPD), a method for learning from offline trajectories using relative step advantages. SAPD decomposes multi-turn trajectories into individual decision contexts for on-policy distillation, allowing the student to generate responses conditioned on recorded histories, and introduces relative step advantage signals to stabilize training. The entire process requires neither new environment observations nor additional multi-turn interactions. Experiments on ALFWorld, WebShop, and Search-based QA show that SAPD improves performance across different teacher configurations, mitigates catastrophic forgetting compared with SFT, and runs at least $4.7\times$ faster per training step than online OPD. We will release our code soon.

==> sapd_frontmatter.tex <==
% Title, author order, affiliations, and footnotes transcribed from
% opd_iclr_2027.pdf, compiled on 2026-10-16. Only layout is changed.

\title{SAPD: Learning from Agent Experience\\
without Environment Interaction}

\author{%
\textbf{Juncheng Diao\textsuperscript{1,2}\thanks{Equal contribution.},
Haibin Wang\textsuperscript{1}\footnotemark[1]\thanks{Corresponding author.},
Wei Shi\textsuperscript{1},
Yifan Ding\textsuperscript{1}}\\[3pt]
\textbf{Qingbin Li\textsuperscript{2},
Rongxiang Weng\textsuperscript{1} \&
Xunliang Cai\textsuperscript{1}}\\[6pt]
\textsuperscript{1}Meituan, LongCat Team\\
\textsuperscript{2}University of Chinese Academy of Sciences\\[3pt]
{\small\texttt{diaojuncheng24@mails.ucas.ac.cn},
\texttt{wanghaibin09@meituan.com}}%
}

\renewcommand{\longcatshorttitle}{SAPD}

